Boolean Abstractions for Realizability Modulo Theories (Extended version)

In this paper, we address the problem of the (reactive) realizability of specifications of theories richer than Booleans, including arithmetic theories. Our approach transforms theory specifications into purely Boolean specifications by (1) substituting theory literals by Boolean variables, and (2) computing an additional Boolean requirement that captures the dependencies between the new variables imposed by the literals. The resulting specification can be passed to existing Boolean off-the-shelf realizability tools, and is realizable if and only if the original specification is realizable. The first contribution is a brute-force version of our method, which requires a number of SMT queries that is doubly exponential in the number of input literals. Then, we present a faster method that exploits a nested encoding of the search for the extra requirement and uses SAT solving for faster traversing the search space and uses SMT queries internally. Another contribution is a prototype in Z3-Python. Finally, we report an empirical evaluation using specifications inspired in real industrial cases. To the best of our knowledge, this is the first method that succeeds in non-Boolean LTL realizability.

==> Appendices/11-extendedPrelims.tex <==
\section{Extended State of the Art} \label{appSec:stateOfArt}

\subsection{Preliminaries} \label{appSubSec:extendedPreliminaries}

%**THIS IS FULLY COPIED FROM SYNT.

We fix an alphabet $\Sigma$ and we call each element $a\in\alphabet$ a
{\em letter}.
%
In case of the Boolean version of the logic, $\AP$ is a set of {\em
  atomic propositions} and $\alphabet=2^\AP$ is the {\em alphabet}.
%
A {\em trace} is an infinite sequence $\sigma=a_0a_1\cdots$ of letters from 
$\alphabet$.
%
We denote the set of all infinite traces by $\alphabet^\omega$.
%
We use $\sigma(i)$ for $a_i$ and $\sigma^i$ for the suffix
$a_ia_{i+1}\cdots$.


\subsubsection{Linear Temporal Logic (LTL)}

Linear temporal logic (LTL) is a modal temporal logic with modalities
referring to time.
%
The syntax of LTL is the following:
 %
\[
  \varphi  ::= T \DefOR a \DefOR \varphi \lor \varphi \DefOR \varphi \land \varphi \DefOR \neg \varphi
  \DefOR \Next \varphi \DefOR \varphi \U\varphi \DefOR \varphi \R\varphi
\]
where $a$ is an atomic proposition, $\lor$, $\land$ and $\neg$ are the
usual Boolean disjunction, conjunction and negation, and $\Next$, $\U$
and $\R$ are the next, until and release temporal operators.
%
The semantics of LTL associate traces $\sigma\in\Sigma^\omega$ with
formulae as follows:
 \[
   \begin{array}{l@{\hspace{0.3em}}c@{\hspace{0.3em}}l}
     \sigma \models T & \text{always} & \\
     \sigma \models a & \text{iff } & a \in\sigma(0) \\
     \sigma \models \varphi_1 \Or \varphi_2 & \text{iff } & \sigma\models \varphi_1 \text{ or } \sigma\models \varphi_2 \\
     \sigma \models \varphi_1 \And \varphi_2 & \text{iff } & \sigma\models \varphi_1 \text{ and } \sigma\models \varphi_2 \\
     \sigma \models \neg \varphi & \text{iff } & \sigma \not\models\varphi \\
     \sigma \models \Next \varphi & \text{iff } & \sigma^1\models \varphi \\
     \sigma \models \varphi_1 \U \varphi_2 & \text{iff } & \text{for some } i\geq 0\;\; \sigma^i\models \varphi_2, \text{ and } \\
                      & & \hspace{2em} \text{for all } 0\leq j<i, \sigma^j\models\varphi_1 \\
     \sigma \models \varphi_1 \R \varphi_2 & \text{iff } & \text{either for all } i\geq 0\;\; \sigma^i\models \varphi_2, \text{ or } \\
                      & & \hspace{1em} \text{for some } i\geq 0\;\; \sigma^i\models\varphi_1 \text{ and } \\
     & & \hspace{2em} \text{for all } 0\geq j\geq i\;\; \sigma^j\models\varphi_2 \\
   \end{array}
 \]
% \[
%   \begin{array}{l@{\hspace{0.5em}}l@{\hspace{0.5em}}l@{\hspace{3.8em}}l@{\hspace{0.3em}}c@{\hspace{0.3em}}l}
%     \sigma \models T & \text{always} & &
%     \sigma \models \varphi_1 \Or \varphi_2 & \text{iff } & \sigma\models \varphi_1 \text{ or } \sigma\models \varphi_2 \\
%     \sigma \models a & \text{iff } & \sigma(0)(a) = \True &
%     \sigma \models \neg \varphi & \text{iff } & \sigma \not\models\varphi \\
%     \sigma \models \Next \varphi & \text{iff } & \sigma^1\models \varphi &&& \\
%     \sigma \models \varphi_1 \U \varphi_2 & \text{iff } & \multicolumn{4}{l}{\text{for some } j\geq 0\;\; \sigma^j\models \varphi_2, \text{and for all } 0\leq i<j, \sigma^i\models\varphi_1}
%   \end{array}
% \]
%
 The set of temporal operators $\Next$, $\U$ and $\R$ is not minimal
 but admits a negation normal form.
 % 
 Common derived operators are $\Event\varphi\DefinedAs T \U\varphi$
 and $\Always\varphi\DefinedAs\Not\Event\Not\varphi$.
 %
 A specification is called a safety specification if it only uses
 $\Next$ and $\Always$ in its negation normal form.

\subsubsection{Reactive synthesis and games}

Synthesis studies automatic generation of state machines from
high-level specifications.

Reactive synthesis
\cite{thomas08church,piteram06synthsis,bloem12synthesis,finkbeiner16synthesis,bloem21vacuity}
is the problem of producing a system from an LTL specification, where
the atomic propositions are split into propositions that are
controlled by the environment and those that are controlled by the
system.

%http://i-cav.org/cavlinks/wp-content/uploads/2019/07/ReactiveSynthesis_Lecture_1.pdf
Synthesis can be seen as a turn-based game, where in each turn the
environment produces values of its variables (inputs) and the
system responds with values of its variables (outputs).
%
A play is an infinite sequence of turns.
%
The system player wins a play according to an LTL formula $\varphi$ if
the trace of the play satisfies $\varphi$.
%
The arena of the game is the history of previous moves.
%
A strategy of a player is a map from the position into a move for the
player.
%
A play is played according to a strategy if all the moves of the
corresponding player are played according to the strategy.
%
A strategy is winning for a player if all the possible plays played
according to the strategy are winning.

In this paper we consider safety games, where the System wins if only
'safe' positions are visited (i.e. if the environment does not reach
an 'unsafe' position).
%

In this paper we consider the synthesis problem for theories, that is,
the set $\AP$ of atomic propositions is literals from some theory.
%
In this case, the alphabet is the possible valuations of the variables
(from the domains of the theories) and the atomic propositions
$a\in\AP$ are evaluated in the corresponding theories.
%
In terms of games, each player chooses in its turn a valuation of the
variables assigned to her.
%
We show in Section~\ref{sec:booleanAbs} a method that
reduces this problem to a purely Boolean synthesis problem.

\subsection{Reactivity Modulo Theories: Related work}

We call the \textit{reactivity modulo theory} to all those approaches that intend to add rich types (theory-based types) to the fields of LTL, reactive synthesis, infinite games and reactive systems overall.

There are many alternatives to LTL for specifying properties of
reactive systems, including
STL~\cite{ramanETAL2015reactiveSynthesisSignalTemporalLogic} and
GTL~\cite{cyrlukNarendran2001groundTemporalLogicHardwareVerification}.
%
We address here LTL with richer theories in the data, including a
large class of first-order theories, which have long been used in
verification
\cite{mannaPnueli1982verificationConcurrentProgramsTemporalProof}.

\subsubsection{Temporal stream logic}

Temporal Stream Logic (TSL) [1], was introduced as a new temporal logic for reactive synthesis that separates control from data. In the original TSL semantics, all functions and predicates are uninterpreted.

The difference with respect to our approach is that, because of the variable update operations TSL allows, its synthesis is undecidable in general, while we are exploring how to improve the limitations but keeping the synthesis problem decidable. In comparison, a limitation of our approach of course is that we cannot compare (rich) values across time which is an important aspect to explore in future work.

In addition, at [2], they extend TSL with first-order theories, enabling them to specify systems using interpreted functions and predicates such as incrementation or equality. They investigate the satisfiability problem of TSL modulo the theory of uninterpreted functions as well as with respect to Presburger arithmetic and the theory of equality: for all three theories, TSL satisfiability is also highly undecidable. Nevertheless, they identify three fragments of TSL for which the satisfiability problem is (semi-)decidable in the theory of uninterpreted functions and present an algorithm – which is not, obviously, guaranteed to terminate – for checking the satisfiability of a TSL formula in the theory of uninterpreted functions. This method scales well.

Also, at [3], they present a synthesis procedure for TSL(T), an extension of TSL with theories (arbitrary decidable theories in which quantifier elimination is possible). Synthesis is performed using a counter-example guided synthesis loop and an LTL synthesis procedure and. This part is similar to our extra requirement approach. Once again, they show that the synthesis problem for TSL(T) is undecidable, but propose a method that can successfully synthesize or show unrealizability of several non-Boolean examples.

\subsubsection{Other \textit{rich} temporal logics}

Another approach is Constraint LTL (CLTL)
\cite{demriDSouza2002automataTheoreticApproachConstraintLTL}, which extends
LTL with the possibility of expressing constraints between variables
at bounded distance (of time).
%
A constraint system $\mathcal{D}$ consists of a concrete domain and an
interpretation of relations on the domain. In Constraint LTL over
$\mathcal{D}$ (CLTL($\mathcal{D}$)), one can relate variables with
relations defined in $\mathcal{D}$. Similar to updates in TSL, CLTL
can specify assignment-like statements by utilizing the equality
relation. Like for all constraints allowing for a counting mechanism,
LTL with Presburger constraints, i.e.,
$\textit{CLTL}(\mathbb{Z}, =, +)$, is undecidable.
%
The difference with respect to our approach is that we do not allow
comparisons (in fact, no type of predicate) of variables within
different timesteps.

\subsubsection{Boolean abstraction-like ideas}

%from: https://dl.acm.org/doi/10.1007/978-3-030-38919-2_14#
In addition, variable automata with arithmetic enable the specification of reactive
systems with variables over an infinite domain of numeric values and
whose operation involves arithmetic manipulation
\cite{faranKupferman2018LTLArithmeticApplicationsReasoningHierarchical}
of these
values. \cite{faranKupferman2020synthesisSpecificationsArithmetic}
studies the synthesis problem for such specifications.

As for works closest to ours, the \cite{cheng2013numerical} preprint
proposes numerical LTL synthesis for cyber-physical systems, whose
calculations involve an interplay between an LTL synthesizer and a
nonlinear real arithmetic theory checker. However, their idea only
considers specifications where the arithmetic predicates belong to the
environment and indeed they \textit{overapproximate} the result.
%
Moreover, \cite{cheng2013numerical} does not contain full results.

Also, the problem of solving linear arithmetic games is addressed in
\cite{azadehKincaid2017strategySynthesisLinearArithmetic}, producing
algorithms for synthesizing winning strategies relying on a dedicated
decision procedure for quantified linear arithmetic formulae. However,
in addition to not being a Booleanization method, but a synthesis
method, they do not consider time modalities either.

\subsubsection{Infinite (state) games}

Since the specification that we will consider model infinite-state games, we also address this state of the art.

Many techniques, both explicit-state \cite{Thomas1995synthesisStrategiesInfiniteGames} and symbolic \cite{piterman06synthesis, hardingETAL2005newAlgorithmStrategySynthesisLTL}, are known for games on finite graphs.
%self
As for infinite-state games, a witness of a recent researches on them
is \cite{baier2021causalitybased} where a causality-based algorithm
for solving two-player reachability games represented by logical
constraints is presented, based on the notion of \textit{subgoals}.

%from: https://arxiv.org/pdf/2105.14247.pdf
Other approaches for solving infinite-state games include symbolic
BDD-based state-space exploration
\cite{edelkamp2002symbolicExplorationTwoPlayerGames}, computing
winning regions of both players using proof rules
\cite{beyeneETAL2014constraintApproachSolvingGamesInfinite} and
predicate abstraction
\cite{walkerRyzhyk2014predicateAbstractionReactiveSynthesis}. There is
also synthesis of infinite-state reactive implementations with random
behavior \cite{katis2020synthesisInfiniteRandom}.

\subsection{Reactivity modulo theories: Our domain} \label{appSubSec:arithmetics}

\subsubsection{Arithmetic first-order theories}

We use sorted first-order theories for extending the expressivity of
the atomic predicates.
%
For our purposes, a (sorted) first-order theory consists of (1) a
first-order vocabulary to form terms and predicates, (2) an
interpretation of the domains of the sorts, and (3) a reasoning system
to decide validity of sentences in the theory.

A particular class of first-order theories is that of arithmetic
theories, which are well studied in mathematics and theoretical
computer science, and are of particular relevance in formal
methods. Thus, even if the Boolean abstraction technique that we present allows any theory that is ddecidable on its $\exists^*\forall^*$ fragment, we are only considering arithmetic specifications in this paper, for illustrative reasons.

Note that all these theories are decidable.

We consider linear (arithmetic) theories:

\begin{itemize}
\item \textit{Linear Natural Arithmetic} or
  $\mathcal{T}_{\mathbb{N}}$ is the theory of natural numbers with
  addition but no arbitrary multiplication
  \cite{presburger1929theoremProving,davis1957presburgerImplementation,stansifer1984presburgersArticle,OPPEN1978upperBoundPresburger}. The
  signature is: $\Sigma_{\mathbb{N}} = \{ 0,1,\ldots,+,=\}$. One example of a
  literal is $(2x=4)$.
\item \textit{Linear Integer Arithmetic} or
  $\mathcal{T}_{\mathbb{Z}}$ the theory of integer numbers with
  addition but no arbitrary multiplication
  \cite{cooper1972theoremProving,Harrison2007IntroductionTL,zoharbradley2007Calculus,fischerRabin1998SuperExponentialComplexityPresburger}. The
  signature is
  $\Sigma_{\mathbb{Z}} = \{\ldots,-1,0,1,\ldots,,+,-,=,>\}$. A
  sentence literal is $(2x=-4)$.
    \item \textit{Linear Rational/Real Arithmetic} or
    $\mathcal{T}_{\mathbb{Q}}$: the theory of real/rational numbers with
    addition but no arbitrary multiplication
    \cite{Robinson1949DefinabilityAD,ferranteRackoff1975TheoryOfRationals,zoharbradley2007Calculus,Voigt2021Decidable}.
    The signature is $\Sigma_{\mathbb{Q}} = \{0,k,+,-,=,>\}$. For
    instance, a valid literal is $(2x=-\frac{1}{3})$.
\end{itemize}

And non-linear theories:

\begin{itemize}
    \item \textit{Nonlinear Real Arithmetic} or
    $\mathcal{T}_{\mathbb{R}}$ is the theory of real numbers with both
    addition and arbitrary multiplication
    \cite{tarski1951decisionElementary,seidenberg1954NewDecisionElementaryAlgebra,collins1975quantifierEliminationRealClosedCylindricalDecomposition,louVanDries1988alfredTarskiReal}.
    %
    The signature is $\Sigma_{\mathbb{R}} = \{0,k,+,-,=,>,\cdot\}$.
    %
    An example of a literal is $(2x^2=\frac{1}{3})$.
    \item Finally, we introduce \textit{Nonlinear Complex Arithmetic}
    or $\mathcal{T}_{\mathbb{C}}$, the theory of complex
    numbers with both addition and arbitrary multiplication
    \cite{ierardi1989quantifierEliminationAlgebraicallyClosed,ierardi1989ComplexityQuantifierEliminationAlgebraically,chistovGrigoriev2006complexityQuantifierEeliminationAlgebraically,harrison2008complexQuantifierHol}.
    %
    The signature is $\Sigma_{\mathbb{C}} = \{0,k,+,-,=,>,\cdot, i\}$. For
    instance, a literal is $(2x^2=-3)$.
\end{itemize}

\subsubsection{Theory-augmented Linear Temporal Logic: \textit{LTL}$_\mathcal{T}$} \label{subSec:LTLt}

We extend LTL by accepting atomic propositions as literals from
theories.
%
We call $\textit{LTL}_{\mathcal{T}}$ to the extension of LTL where
there is a set of literals that are part of a first-order theory
$\mathcal{T}$.
%
In the realizability problem where theories are involved, the
variables that occur in the literals in the specification formula
$\varphi$ are split into those variables controlled by the environment
($\overline{v}_e$) and those controlled by the system
($\overline{v}_s$).
%
Thus, we have formulae $\varphi[\overline{v}_e, \overline{v}_s]$,
where $\overline{v}_e \cap \overline{v}_s = \emptyset$ and both if
$ v_e \in \overline{v}_e$ and $ v_s \in \overline{v}_s$, then
$v_e, v_s \in \mathcal{T}$.
%
Note that alphabet $\Sigma$ is now a valuation of the variables in
$\overline{v}_e$ and $\overline{v}_s$.
%
A trace is now an infinite sequence of valuations of the variables,
which induces an infinite sequence of Boolean values of the literals
that occurring in the specification, which in turn provide a valuation
of the formulae against the traces.

The realizability problem from an $\textit{LTL}_{\mathcal{T}}$
corresponds, in general, to a game with an infinite arena (and where
positions may have infinitely many successor if the ranges of the
variables controlled by the system and the environment are infinite).
%
For instance, consider an example formula from
$\textit{LTL}_{\mathbb{R}}$: $((x>1) \rightarrow \Next(y>x))$,
where $ x \in \overline{v}_e \wedge x: \mathbb{R}$ and
$ y \in \overline{v}_s \wedge y: \mathbb{R}$.
%
At time $0$, the environment may choose $\overline{v}_e^0=\{x^0=2\}$
environment valuation in timestep $0$, and the system may respond with
$\overline{v}_s^0=\{y^0=2\}$, with $\overline{v}_s^0=\{y^0=3\}$.
%
In this case, the choice $y^0=2$ makes the formula false so the
environment would win the play.

%As said, we are only considering arithmetic theories $\mathcal{T}_{\mathbb{N}}$, $\mathcal{T}_{\mathbb{Z}}$, $\mathcal{T}_{\mathbb{Q}}$, $\mathcal{T}_{\mathbb{R}}$, $\mathcal{T}_{\mathbb{C}}$ as $\mathcal{T}$.

==> Appendices/13-semanticsLTL.tex <==
\section{Semantics of LTL}

The semantics of LTL associate traces $\sigma\in\Sigma^\omega$ with
formulae as follows:
 \[
   \begin{array}{l@{\hspace{0.3em}}c@{\hspace{0.3em}}l}
     \sigma \models T & \text{always} & \\
     \sigma \models a & \text{iff } & a \in\sigma(0) \\
     \sigma \models \varphi_1 \Or \varphi_2 & \text{iff } & \sigma\models \varphi_1 \text{ or } \sigma\models \varphi_2 \\
     \sigma \models \varphi_1 \And \varphi_2 & \text{iff } & \sigma\models \varphi_1 \text{ and } \sigma\models \varphi_2 \\
     \sigma \models \neg \varphi & \text{iff } & \sigma \not\models\varphi \\
     \sigma \models \Next \varphi & \text{iff } & \sigma^1\models \varphi \\
     \sigma \models \varphi_1 \U \varphi_2 & \text{iff } & \text{for some } i\geq 0\;\; \sigma^i\models \varphi_2, \text{ and } \\
                      & & \hspace{2em} \text{for all } 0\leq j<i, \sigma^j\models\varphi_1 \\
     \sigma \models \varphi_1 \R \varphi_2 & \text{iff } & \text{either for all } i\geq 0\;\; \sigma^i\models \varphi_2, \text{ or } \\
                      & & \hspace{1em} \text{for some } i\geq 0\;\; \sigma^i\models\varphi_1 \text{ and } \\
     & & \hspace{2em} \text{for all } 0\geq j\geq i\;\; \sigma^j\models\varphi_2 \\
   \end{array}
 \]
%
 The set of temporal operators $\Next$, $\U$ and $\R$ is not minimal
 but admits a negation normal form.
 % 
 Common derived operators are $\Event\varphi\DefinedAs T \U\varphi$
 and $\Always\varphi\DefinedAs\Not\Event\Not\varphi$.
 %
 A specification is called a safety specification if it only uses
 $\Next$ and $\Always$ in its negation normal form.
 %
 In this paper we consider standard (future) LTL, and no variation of this one, such as Past LTL~\cite{Gabbay1980OnTT}.


==> Appendices/7-algorithmsDepth.tex <==
\section{Algorithms unrolled}

Note the \textit{for} loop in the Alg~\ref{algoBruteForce} and the \textit{while} loop in Alg~\ref{algoModelLoop}.

\begin{algorithm}
\SetAlgoLined
\textbf{Input: }$\phiT$\;
$\varphi'\gets \phiT[l_i \leftarrow s_i]$;  \textit{VR} $\gets$ \{\}\;
$\calC \gets \textit{choices}(\textit{literals}(\phiT))$;
$\calR \gets 2^{\calC}$\;
%$\textit{VR} \gets \emptyset$\;
 \For{$(P,A) \in \calR$}{
   \If{$\exists\xs.\react_{(P,A)}(\xs)$ is valid}
   {
     $\textit{VR} \gets \textit{VR} \cup \{ (P,A) \}$\;
    }
 }
 $\displaystyle\phiExtra \gets \bigwedge_{(P,A)\in \textit{VR}} (e_{(P,A)} \rightarrow \bigvee_{c\in P} (\bigwedge_{l_i\in c}s_i\wedge \bigwedge_{l_i\notin c}\neg s_i))$ \;
 $\phiB \gets \varphi' \wedge \phiExtra$ \;
 \Return $\phiB$
 \caption{Brute-force Boolean Abstraction algorithm}
 \label{algoBruteForce}
\end{algorithm}

%\subsubsection{Model Loop algorithm} Note the \textit{while} loop.

\begin{algorithm}[H] \label{algoModelLoop}
\SetAlgoLined
\textbf{Input: }$\phiT$\;
$\varphi'\gets \phiT[l_i \leftarrow s_i]$;  \textit{VR} $\gets$ \{\}\;
$\calC \gets \textit{choices}(\textit{literals}(\phiT))$;
$\calR \gets 2^{\calC}$\;
 $\overline{c} \gets$ From  $\{\mathcal{C}, \mathcal{P}, \mathcal{A}\}$ obtain Boolean configurations, where $c \in \overline{c} \equiv p \in \mathcal{P}$ and $\neg c \in \overline{c} \equiv a \in \mathcal{A}$ \;
 $\varphi = \exists \overline{c} \textit{. } \neg(\bigwedge_{0 \leq i \leq |\overline{c}|} \neg c_i) $\;
 \While{$\textit{SAT}(\varphi)$}{
    $m = model(\varphi)$\;
    $t = translate\_toTheory(m)$\; %\#For instance, from $c_0 \neg c_1 \neg c_2 c_3$ to \textit{PAAP}. 
    \If{$\exists \overline{x} :: (t)$ is valid}{
    $pos = take\_Positives(t)$ \;
    $\varphi = \varphi \wedge \neg(\bigwedge_{0 \leq j \leq |pos|} \neg pos_j)$ \;
    \textit{VR} $\gets$ \textit{VR} $\cup$ $(e_{\textit{t}}, pots(t))$\;
    %(i.e. Add: $fresh(\overline{e}) \implies Pots\_of(React_i)$) 
    }
    \Else{
    $neg = take\_Negatives(t)$ \;
    $\varphi = \varphi \wedge \neg(\bigwedge_{0 \leq k \leq |neg|} \neg neg_k)$ \;
    }
 }
 $\displaystyle\phiExtra \gets \bigwedge_{(P,A)\in \textit{VR}} (e_{(P,A)} \rightarrow \bigvee_{c\in P} (\bigwedge_{l_i\in c}s_i\wedge \bigwedge_{l_i\notin c}\neg s_i))$ \;
 %$\varphi^{extra} \gets get\_minimal(\varphi^{extra})$ \;
 $\phiB \gets \varphi' \wedge \phiExtra$ \;
 \Return $\varphi^{\mathbb{B}}$
 \caption{Model-loop based Boolean Abstraction algorithm}
\end{algorithm}

\pagebreak

Note the heuristics in Alg. \ref{algoDefinitive}.

\begin{algorithm}[H] \label{algoDefinitive}
\SetAlgoLined
\textbf{Input: }$\phiT$\;
 \textit{fatigue}, \textit{division} \#These are (1) the fixed number of inner-loops and (2) if UNSAT outer model is divisible by this number, we enter inner-loop \;
 $\mathcal{S} \gets  get\_clusters(\textit{all\_literals})$ \;
 $\varphi^{extra} \gets \top$ \;
 \For{$s \in \mathcal{S}$}{
    $\varphi^{''} \gets \{\}$ \;
    $\overline{l} \gets get\_literals(\mathcal{S})$ \#Cluster's literals \;
    \For {$0<r<|\overline{l}|$}{
     $\varphi^{''} \gets \varphi^{''} \cup \varphi^{Num}[l_r \leftarrow s_r]$ \;
    }
     $\mathcal{C} \gets$ obtain\_the\_configutations\_from\_the\_literals\;
     $(\mathcal{P}, \mathcal{A}) \gets$ From $\mathcal{C}$, compute the sets of potentials and antipotentials \; 
     $\overline{c} \gets$ From  $\{\mathcal{C}, \mathcal{P}, \mathcal{A}\}$ obtain Boolean configurations, where $c \in \overline{c} \equiv p \in \mathcal{P}$ and $\neg c \in \overline{c} \equiv a \in \mathcal{A}$ \;
     Valid $\gets$ \{\}\;
     $num\_unsats \gets 0$ \;
     $\varphi = \exists \overline{c} \textit{. } \neg(\bigwedge_{0 \leq i \leq |\overline{c}|} \neg c_i) $\;
     \While{$\textit{SAT}(\varphi)$}{
        $t = translate\_toTheory(model(\varphi))$\;
        %$t = translate\_toTheory(m)$\; %\#For instance, from $c_0 \neg c_1 \neg c_2 c_3$ to \textit{PAAP}. 
        \If{$\exists \overline{x} :: (t)$ is valid}{
        $pos = take\_Positives(t)$ \;
        $\varphi = \varphi \wedge \neg(\bigwedge_{0 \leq j \leq |pos|} \neg pos_j)$ \;
        Valid $\gets$ Valid $\cup$ $(e_{\textit{t}}, pots(t))$\;
        %(i.e. Add: $fresh(\overline{e}) \implies Pots\_of(React_i)$) 
        }
        \Else{
        $neg = take\_Negatives(t)$ \;
        $\varphi = \varphi \wedge \neg(\bigwedge_{0 \leq k \leq |neg|} \neg neg_k)$ \;
        
            \If{$num\_unsats \% division = 0$}{
                $also\_cut = inner\_loop (t, \textit{fatigue})$ \; 
                $\varphi = \varphi \wedge \neg(\bigwedge_{0 \leq w \leq |also\_cut|} \neg also\_cut_w)$ \
            }
        $num\_unsats = num\_unsats + 1$
        }
     }
 $\displaystyle \varphi^{extra}_s \gets \bigwedge_{(P,A)\in \textit{VR}} (e_{(P,A)} \rightarrow \bigvee_{c\in P} (\bigwedge_{l_i\in c}s_i\wedge \bigwedge_{l_i\notin c}\neg s_i))$ \;
     %$\varphi^{extra}_s \gets get\_minimal(\varphi^{extra}_s)$ \;
     $\varphi^{extra} = \varphi^{extra} \wedge \varphi^{extra}_s$
    }

 $\phiB \gets \varphi' \wedge \phiExtra$ \;
 \Return $\varphi^{\mathbb{B}}$
 \caption{Double SAT algorithm with heuristics}
\end{algorithm}


==> Appendices/7-supportMaterial.tex <==
\section{Extra support material}

This section elaborates on the procedures presented (with algorithms) and the empirical evaluation (with tables). It is recommendable, yet not essential, to better understand the results.

\subsection{Algorithms in depth}

For the theoretical development (i.e., Section 3).

\begin{algorithm}
\SetAlgoLined
\textbf{Input: }$\phiT$\;
$\varphi'\gets \phiT[l_i \leftarrow s_i]$\;
$\calC \gets \textit{confs}(\textit{literals}(\phiT))$\;
$\calR \gets 2^{\calC}$\;
$\textit{VR} \gets \emptyset$\;
 \For{$(P,A) \in \calR$}{
   \If{$\exists\xs.\react_{(P,A)}(\xs)$ is valid}
   {
     $\textit{VR} \gets \textit{VR} \cup \{ (P,A) \}$\;
    }
 }
 $\displaystyle\phiExtra \gets \bigwedge_{(P,A)\in \textit{VR}} (e_{(P,A)} \rightarrow \bigvee_{c\in P} (\bigwedge_{l_i\in c}s_i\wedge \bigwedge_{l_i\notin c}\neg s_i))$ \;
 $\phiB \gets \varphi' \wedge \phiExtra$ \;
 \Return $\phiB$
 \caption{Brute-force Boolean Abstraction algorithm}
 \label{algoBruteForce}
\end{algorithm}

\begin{algorithm}[H] \label{algoModelLoop}
\SetAlgoLined
$\varphi'\gets \phiT[l_i \leftarrow s_i]$\;
 $\mathcal{C} \gets$ obtain\_the\_configutations\_from\_the\_literals\;
 $(\mathcal{P}, \mathcal{A}) \gets$ From $\mathcal{C}$, compute the sets of potentials and antipotentials \; 
 $\overline{c} \gets$ From  $\{\mathcal{C}, \mathcal{P}, \mathcal{A}\}$ obtain Boolean configurations, where $c \in \overline{c} \equiv p \in \mathcal{P}$ and $\neg c \in \overline{c} \equiv a \in \mathcal{A}$ \;
 Valid $\gets$ \{\}\;
 $\varphi = \exists \overline{c} \textit{. } \neg(\bigwedge_{0 \leq i \leq |\overline{c}|} \neg c_i) $\;
 \While{$\textit{SAT}(\varphi)$}{
    $m = model(\varphi)$\;
    $t = translate\_toTheory(m)$\; %\#For instance, from $c_0 \neg c_1 \neg c_2 c_3$ to \textit{PAAP}. 
    \If{$\exists \overline{x} :: (t)$ is valid}{
    $pos = take\_Positives(t)$ \;
    $\varphi = \varphi \wedge \neg(\bigwedge_{0 \leq j \leq |pos|} \neg pos_j)$ \;
    Valid $\gets$ Valid $\cup$ $(e_{\textit{t}}, pots(t))$\;
    %(i.e. Add: $fresh(\overline{e}) \implies Pots\_of(React_i)$) 
    }
    \Else{
    $neg = take\_Negatives(t)$ \;
    $\varphi = \varphi \wedge \neg(\bigwedge_{0 \leq k \leq |neg|} \neg neg_k)$ \;
    }
 }
 $\displaystyle\phiExtra \gets \bigwedge_{(P,A)\in \textit{VR}} (e_{(P,A)} \rightarrow \bigvee_{c\in P} (\bigwedge_{l_i\in c}s_i\wedge \bigwedge_{l_i\notin c}\neg s_i))$ \;
 %$\varphi^{extra} \gets get\_minimal(\varphi^{extra})$ \;
 $\phiB \gets \varphi' \wedge \phiExtra$ \;
 \Return $\varphi^{\mathbb{B}}$
 \caption{Model-loop based Boolean Abstraction algorithm}
\end{algorithm}

\begin{algorithm}[H] \label{algoDoubleSAT}
\SetAlgoLined
$\varphi'\gets \phiT[l_i \leftarrow s_i]$\;
 $\mathcal{C} \gets$ obtain\_the\_configutations\_from\_the\_literals\;
 $(\mathcal{P}, \mathcal{A}) \gets$ From $\mathcal{C}$, compute the sets of potentials and antipotentials \; 
 $\overline{c} \gets$ From  $\{\mathcal{C}, \mathcal{P}, \mathcal{A}\}$ obtain Boolean configurations, where $c \in \overline{c} \equiv p \in \mathcal{P}$ and $\neg c \in \overline{c} \equiv a \in \mathcal{A}$ \;
 Valid $\gets$ \{\}\;
 $\varphi = \exists \overline{c} \textit{. } \neg(\bigwedge_{0 \leq i \leq |\overline{c}|} \neg c_i) $\;
 \While{$\textit{SAT}(\varphi)$}{
    $m = model(\varphi)$\;
    $t = translate\_toTheory(m)$\; %\#For instance, from $c_0 \neg c_1 \neg c_2 c_3$ to \textit{PAAP}. 
    \If{$\exists \overline{x} :: (t)$ is valid}{
    $pos = take\_Positives(t)$ \;
    $\varphi = \varphi \wedge \neg(\bigwedge_{0 \leq j \leq |pos|} \neg pos_j)$ \;
    Valid $\gets$ Valid $\cup$ $(e_{\textit{t}}, pots(t))$\;
    %(i.e. Add: $fresh(\overline{e}) \implies Pots\_of(React_i)$) 
    }
    \Else{
    $neg = take\_Negatives(t)$ \;
    $\varphi = \varphi \wedge \neg(\bigwedge_{0 \leq k \leq |neg|} \neg neg_k)$ \;
    $also\_cut = inner\_loop (t)$ \; 
    \# We prune here all the space that the inner loop offers to cut.
    $\varphi = \varphi \wedge \neg(\bigwedge_{0 \leq w \leq |also\_cut|} \neg also\_cut_w)$ \;
    }
 }
 $\displaystyle\phiExtra \gets \bigwedge_{(P,A)\in \textit{VR}} (e_{(P,A)} \rightarrow \bigvee_{c\in P} (\bigwedge_{l_i\in c}s_i\wedge \bigwedge_{l_i\notin c}\neg s_i))$ \;
 %$\varphi^{extra} \gets get\_minimal(\varphi^{extra})$ \;
 $\phiB \gets \varphi' \wedge \phiExtra$ \;
 \Return $\varphi^{\mathbb{B}}$
 \caption{Double-SAT based Boolean Abstraction algorithm}
\end{algorithm}

\begin{algorithm}[H] \label{algoDefinitive}
\SetAlgoLined
 \textit{fatigue} \#This is the fixed number of inner-loops \;
 $division$ \#If the UNSAT outer model is divisible by this number, we enter the inner loop \;
 $\mathcal{S} \gets  get\_clusters(\textit{all\_literals})$ \;
 $\varphi^{extra} \gets \top$ \;
 \For{$s \in \mathcal{S}$}{
    $\varphi^{booleanized} \gets \{\}$ \;
    $\overline{l} \gets get\_literals(\mathcal{S})$ \#Cluster's literals \;
    \For {$0<r<|\overline{l}|$}{
     $\varphi^{booleanized} \gets \varphi^{booleanized} \cup \varphi^{Num}[l_r \leftarrow s_r]$ \;
    }
     $\mathcal{C} \gets$ obtain\_the\_configutations\_from\_the\_literals\;
     $(\mathcal{P}, \mathcal{A}) \gets$ From $\mathcal{C}$, compute the sets of potentials and antipotentials \; 
     $\overline{c} \gets$ From  $\{\mathcal{C}, \mathcal{P}, \mathcal{A}\}$ obtain Boolean configurations, where $c \in \overline{c} \equiv p \in \mathcal{P}$ and $\neg c \in \overline{c} \equiv a \in \mathcal{A}$ \;
     Valid $\gets$ \{\}\;
     $num\_unsats \gets 0$ \;
     $\varphi = \exists \overline{c} \textit{. } \neg(\bigwedge_{0 \leq i \leq |\overline{c}|} \neg c_i) $\;
     \While{$\textit{SAT}(\varphi)$}{
        $m = model(\varphi)$\;
        $t = translate\_toTheory(m)$\; %\#For instance, from $c_0 \neg c_1 \neg c_2 c_3$ to \textit{PAAP}. 
        \If{$\exists \overline{x} :: (t)$ is valid}{
        $pos = take\_Positives(t)$ \;
        $\varphi = \varphi \wedge \neg(\bigwedge_{0 \leq j \leq |pos|} \neg pos_j)$ \;
        Valid $\gets$ Valid $\cup$ $(e_{\textit{t}}, pots(t))$\;
        %(i.e. Add: $fresh(\overline{e}) \implies Pots\_of(React_i)$) 
        }
        \Else{
        $neg = take\_Negatives(t)$ \;
        $\varphi = \varphi \wedge \neg(\bigwedge_{0 \leq k \leq |neg|} \neg neg_k)$ \;
        
            \If{$num\_unsats \% division = 0$}{
                $also\_cut = inner\_loop (t, \textit{fatigue})$ \; 
                $\varphi = \varphi \wedge \neg(\bigwedge_{0 \leq w \leq |also\_cut|} \neg also\_cut_w)$ \
            }
        $num\_unsats = num\_unsats + 1$
        }
     }
 $\displaystyle\phiExtra \gets \bigwedge_{(P,A)\in \textit{VR}} (e_{(P,A)} \rightarrow \bigvee_{c\in P} (\bigwedge_{l_i\in c}s_i\wedge \bigwedge_{l_i\notin c}\neg s_i))$ \;
     %$\varphi^{extra}_s \gets get\_minimal(\varphi^{extra}_s)$ \;
     $\varphi^{extra} = \varphi^{extra} \wedge \varphi^{extra}_s$
    }

 $\phiB \gets \varphi' \wedge \phiExtra$ \;
 \Return $\varphi^{\mathbb{B}}$
 \caption{Definitive optimized Boolean Abstraction algorithm}
\end{algorithm}

\subsection{Tables}

For the empirical evaluation (i.e., Section 4).

\subsubsection{Synthetic tests}

We offer results of each test using its best heuristic-setup:

//SEVEN TABLES

\subsubsection{How we found the best heuristic-setups}

In order to discover the best heuristic-setups (at least for these datasets), we made a random search in a hyperparameter search-like idea:

In this paper, we offer a snapshot of it. Concretely, with test 0, we offer how we reached the best heuristic-setups for low cases (less than 5 literals), whereas with test N we show how we reached the best heuristic-setups for higher cases (greater than 4 literals).

//TWO TABLES

\subsubsection{Synthetic tests vs different theories}

We compare each test with the best heuristic-setup of previous section, against different theories.

Note that, in each test, one of the three theories corresponds to the original theory of the test, so each table is comparing the original theory against two modifications.

Test 0:

\begin{center} \label{tablTest0Theories}
\begin{tabular}{||c c c c||} 
 \hline
 Size version & $\mathcal{T}_{\mathbb{N}}$ & $\mathcal{T}_{\mathbb{Z}}$ & $\mathcal{T}_{\mathbb{R}}$ \\ 
 (literals) & (time) & (time) & (time) \\
  & (inner / outer) & (inner / outer) & (inner / outer) \\ [0.5ex] 
 \hline\hline
 2 & 30 & 60 & a\\ 
  & & 900 & a\\
 \hline
 3 & 30 & 16 & a \\
   &  & 30 & a \\
 \hline
 4 & 5 &  10 & a \\
 &  & 10 & a \\
 \hline
 5 & 3 &  4 & a \\
  &  & 3 & a \\
 \hline
 6 & 3 &  4 & a \\
  &  & 3 & a \\
 \hline
 7 & 3 &  4 & a \\
  & & 3 & a \\
 \hline
 8 & 3 &  4 & a \\
  & & 3 & a \\
 \hline
\end{tabular}
\end{center}

Test 1:

\begin{center} \label{tablTest0Theories}
\begin{tabular}{||c c c c||} 
 \hline
 Size version & $\mathcal{T}_{\mathbb{N}}$ & $\mathcal{T}_{\mathbb{Z}}$ & $\mathcal{T}_{\mathbb{R}}$ \\ 
 (literals) & (time) & (time) & (time) \\
  & (inner / outer) & (inner / outer) & (inner / outer) \\ [0.5ex] 
 \hline\hline
 2 & 30 & 60 & a\\ 
  & & 900 & a\\
 \hline
 3 & 30 & 16 & a \\
   &  & 30 & a \\
 \hline
 4 & 5 &  10 & a \\
 &  & 10 & a \\
 \hline
 5 & 3 &  4 & a \\
  &  & 3 & a \\
 \hline
 6 & 3 &  4 & a \\
  &  & 3 & a \\
 \hline
 7 & 3 &  4 & a \\
  & & 3 & a \\
 \hline
 8 & 3 &  4 & a \\
  & & 3 & a \\
 \hline
\end{tabular}
\end{center}

Test 2:

\begin{center} \label{tablTest0Theories}
\begin{tabular}{||c c c c||} 
 \hline
 Size version & $\mathcal{T}_{\mathbb{N}}$ & $\mathcal{T}_{\mathbb{Z}}$ & $\mathcal{T}_{\mathbb{R}}$ \\ 
 (literals) & (time) & (time) & (time) \\
  & (inner / outer) & (inner / outer) & (inner / outer) \\ [0.5ex] 
 \hline\hline
 2 & 30 & 60 & a\\ 
  & & 900 & a\\
 \hline
 3 & 30 & 16 & a \\
   &  & 30 & a \\
 \hline
 4 & 5 &  10 & a \\
 &  & 10 & a \\
 \hline
 5 & 3 &  4 & a \\
  &  & 3 & a \\
 \hline
 6 & 3 &  4 & a \\
  &  & 3 & a \\
 \hline
 7 & 3 &  4 & a \\
  & & 3 & a \\
 \hline
 8 & 3 &  4 & a \\
  & & 3 & a \\
 \hline
\end{tabular}
\end{center}

Test 3:

\begin{center} \label{tablTest0Theories}
\begin{tabular}{||c c c c||} 
 \hline
 Size version & $\mathcal{T}_{\mathbb{N}}$ & $\mathcal{T}_{\mathbb{Z}}$ & $\mathcal{T}_{\mathbb{R}}$ \\ 
 (literals) & (time) & (time) & (time) \\
  & (inner / outer) & (inner / outer) & (inner / outer) \\ [0.5ex] 
 \hline\hline
 2 & 30 & 60 & a\\ 
  & & 900 & a\\
 \hline
 3 & 30 & 16 & a \\
   &  & 30 & a \\
 \hline
 4 & 5 &  10 & a \\
 &  & 10 & a \\
 \hline
 5 & 3 &  4 & a \\
  &  & 3 & a \\
 \hline
 6 & 3 &  4 & a \\
  &  & 3 & a \\
 \hline
 7 & 3 &  4 & a \\
  & & 3 & a \\
 \hline
 8 & 3 &  4 & a \\
  & & 3 & a \\
 \hline
\end{tabular}
\end{center}

Test 4:

\begin{center} \label{tablTest0Theories}
\begin{tabular}{||c c c c||} 
 \hline
 Size version & $\mathcal{T}_{\mathbb{N}}$ & $\mathcal{T}_{\mathbb{Z}}$ & $\mathcal{T}_{\mathbb{R}}$ \\ 
 (literals) & (time) & (time) & (time) \\
  & (inner / outer) & (inner / outer) & (inner / outer) \\ [0.5ex] 
 \hline\hline
 2 & 30 & 60 & a\\ 
  & & 900 & a\\
 \hline
 3 & 30 & 16 & a \\
   &  & 30 & a \\
 \hline
 4 & 5 &  10 & a \\
 &  & 10 & a \\
 \hline
 5 & 3 &  4 & a \\
  &  & 3 & a \\
 \hline
 6 & 3 &  4 & a \\
  &  & 3 & a \\
 \hline
 7 & 3 &  4 & a \\
  & & 3 & a \\
 \hline
 8 & 3 &  4 & a \\
  & & 3 & a \\
 \hline
\end{tabular}
\end{center}

Test 5:

\begin{center} \label{tablTest0Theories}
\begin{tabular}{||c c c c||} 
 \hline
 Size version & $\mathcal{T}_{\mathbb{N}}$ & $\mathcal{T}_{\mathbb{Z}}$ & $\mathcal{T}_{\mathbb{R}}$ \\ 
 (literals) & (time) & (time) & (time) \\
  & (inner / outer) & (inner / outer) & (inner / outer) \\ [0.5ex] 
 \hline\hline
 2 & 30 & 60 & a\\ 
  & & 900 & a\\
 \hline
 3 & 30 & 16 & a \\
   &  & 30 & a \\
 \hline
 4 & 5 &  10 & a \\
 &  & 10 & a \\
 \hline
 5 & 3 &  4 & a \\
  &  & 3 & a \\
 \hline
 6 & 3 &  4 & a \\
  &  & 3 & a \\
 \hline
 7 & 3 &  4 & a \\
  & & 3 & a \\
 \hline
 8 & 3 &  4 & a \\
  & & 3 & a \\
 \hline
\end{tabular}
\end{center}

Test 6:

\begin{center} \label{tablTest0Theories}
\begin{tabular}{||c c c c||} 
 \hline
 Size version & $\mathcal{T}_{\mathbb{N}}$ & $\mathcal{T}_{\mathbb{Z}}$ & $\mathcal{T}_{\mathbb{R}}$ \\ 
 (literals) & (time) & (time) & (time) \\
  & (inner / outer) & (inner / outer) & (inner / outer) \\ [0.5ex] 
 \hline\hline
 2 & 30 & 60 & a\\ 
  & & 900 & a\\
 \hline
 3 & 30 & 16 & a \\
   &  & 30 & a \\
 \hline
 4 & 5 &  10 & a \\
 &  & 10 & a \\
 \hline
 5 & 3 &  4 & a \\
  &  & 3 & a \\
 \hline
 6 & 3 &  4 & a \\
  &  & 3 & a \\
 \hline
 7 & 3 &  4 & a \\
  & & 3 & a \\
 \hline
 8 & 3 &  4 & a \\
  & & 3 & a \\
 \hline
\end{tabular}
\end{center}

Test 7:

\begin{center} \label{tablTest0Theories}
\begin{tabular}{||c c c c||} 
 \hline
 Size version & $\mathcal{T}_{\mathbb{N}}$ & $\mathcal{T}_{\mathbb{Z}}$ & $\mathcal{T}_{\mathbb{R}}$ \\ 
 (literals) & (time) & (time) & (time) \\
  & (inner / outer) & (inner / outer) & (inner / outer) \\ [0.5ex] 
 \hline\hline
 2 & 30 & 60 & a\\ 
  & & 900 & a\\
 \hline
 3 & 30 & 16 & a \\
   &  & 30 & a \\
 \hline
 4 & 5 &  10 & a \\
 &  & 10 & a \\
 \hline
 5 & 3 &  4 & a \\
  &  & 3 & a \\
 \hline
 6 & 3 &  4 & a \\
  &  & 3 & a \\
 \hline
 7 & 3 &  4 & a \\
  & & 3 & a \\
 \hline
 8 & 3 &  4 & a \\
  & & 3 & a \\
 \hline
\end{tabular}
\end{center}

\subsubsection{Industrial tests}

We can see results cluster by cluster.

Case 1: Lift.

\begin{center} \label{tablLift}
\begin{tabular}{||c c c c c||} 
 \hline
 Cluster & Fix & Mod & Time & Quality \\ 
 (vars / lits) & (3 to 100) & (1,2,3 or 4) & (s) & (inner / outer) \\ [0.5ex] 
 \hline\hline
 $Cl_1$ & 30 & 2 & 32.38 &  60 \\ 
  (1, 7) &  &  & & 900 \\
 \hline
 $Cl_2$ & 30 & 2 & 1.27 &  16 \\
  (2, 4) &  &  & & 30 \\
 \hline
 $Cl_3$ & 5 & 2 & 0.57 &  10 \\
 (1, 3) &  &  & & 10 \\
 \hline
 $Cl_4$ & 3 & 2 & 0.23 &  4 \\
 (1, 2) &  &  & & 3 \\
 \hline
\end{tabular}
\end{center}

Case 2: Train


\begin{center} \label{tablTrain}
\begin{tabular}{||c c c c c||} 
 \hline
 Cluster & Fix & Mod & Time & Quality \\ 
 (vars / lits) & (3 to 100) & (1,2,3 or 4) & (s) & (inner / outer) \\ [0.5ex] 
 \hline\hline
 $Cl_1$ & 30 & 2 & 2.33 &  26 \\ 
 (1, 3) &  &  & & 60 \\
 \hline
 $Cl_2$ & 30 & 2 & 0.11 &  2 \\
  (2, 1) &  &  & & 0 \\
 \hline
 $Cl_3$  & 30 & 2 & 0.29 &  2 \\
 (1, 3) &  &  & & 13 \\
 \hline
 $Cl_4$ & 30 & 2 & 0.23 &  3 \\
 (1, 1) &  &  & & 2 \\
 \hline
 $Cl_{5.1}$ & 30 & 2 & 833.32 &  1620 \\
 (3, 6) &  &  & & 9199 \\
 \hline
 $Cl_{5.2}$ & 30 & 2 & EXEC &  EXEC \\
 (4, 6) &  &  & & EXEC \\
 \hline
 $Cl_{6.1}$ & 30 & 2 & EXEC &  EXEC \\
 (2, 4)  &  &  & & EXEC \\
 \hline
 $Cl_{6.2}$ & 30 & 2 & 6571.9738 &  2728 \\
 (3, 12) &  &  & & 40920 \\
 \hline
\end{tabular}
\end{center}

Case 3: Connect

\begin{center} \label{tablConnect}
\begin{tabular}{||c c c c c||} 
 \hline
 Cluster & Fix & Mod & Time & Quality \\ 
 (vars / lits) & (3 to 100) & (1,2,3 or 4) & (s) & (inner / outer) \\ [0.5ex] 
 \hline\hline
 $Cl_{\textit{unique}}$ & 30 & 2 & 0.12 &  4 \\ 
  (2, 2) &  &  & & 0 \\
 \hline
\end{tabular}
\end{center}

Case 4: Cooker

\begin{center} \label{tablCooker}
\begin{tabular}{||c c c c c||} 
 \hline
 Cluster & Fix & Mod & Time & Quality \\ 
 (vars / lits) & (3 to 100) & (1,2,3 or 4) & (s) & (inner / outer) \\ [0.5ex] 
 \hline\hline
 $Cl_{\textit{unique}}$ & 30 & 2 & 2.82 &  8 \\ 
  (3, 5) &  &  & & 120 \\
 \hline
\end{tabular}
\end{center}

Cooker has been a good showing of how different SAT-paths yield totally different performances: there have been other paths: from 7 seconds with (18+270) to 200 seconds with (3853+270), all of them with the same heuristic-setup.

Case 5: (Two) Tanks

//The most complex one

Case 6: Usb

\begin{center} \label{tablUSB}
\begin{tabular}{||c c c c c||} 
 \hline
 Cluster & Fix & Mod & Time & Quality \\ 
 (vars / lits) & (3 to 100) & (1,2,3 or 4) & (s) & (inner / outer) \\ [0.5ex] 
 \hline\hline
 $Cl_{\textit{unique}}$ & 30 & 2 & 0.26 &  8 \\ 
  (2, 3) &  &  & & 0 \\
 \hline
\end{tabular}
\end{center}

Also tested a (synthetic) modification with (3, 5), in 1390.75 seconds and (18038+0) queries.

Case 7: Stages

\begin{center} \label{tablStages}
\begin{tabular}{||c c c c c||} 
 \hline
 Cluster & Fix & Mod & Time & Quality \\ 
 (vars / lits) & (3 to 100) & (1,2,3 or 4) & (s) & (inner / outer) \\ [0.5ex] 
 \hline\hline
 $Cl_A$ & 30 & 2 & 34.25 &  256 \\ 
 (8, 8) &  &  & & 0 \\
 \hline
 $Cl_B$ & 30 & 2 & 2895.74 &  25216 \\
 (8, 11) &  &  & & 2790 \\
 \hline
\end{tabular}
\end{center}

Note that Booleanization has worked so well that they have even wrapped real clusters 1 and 2 into cluster A and wrapped real clusters 3 and 4 into cluster B. This is an example of how a simple coupling (in this case, a single player) yields a simpler Boolean abstractions (and, potentially, a simple synthesis).

\subsubsection{Percentages of coverage}

Here we show the most interesting percentages of coverage in each literal amount, from 2 to 12. Concretely, we show the number of outer+inner queries compared to the total number of queries that would be necessary in an exhaustive-like algorithm. We also show which test yields each result.

\begin{itemize}
    \item $2$ literals, $106.666$\% of queries. Concretely: 
    \begin{itemize}
        \item ($4+14$) out of 15.
    \end{itemize}
    \item 3 literals, 44.705\% of queries:
    \begin{itemize}
        \item ($10+104$) out of 255.
    \end{itemize}
    \item 4 literals, 0.70649271381704\% of queries. Concretely: 
    \begin{itemize}
        \item ($83+380$) out of 65535.
    \end{itemize}
    \item 5 literals, 0.00007203780116\% of queries. Concretely: 
    \begin{itemize}
        \item ($334+2760$) out of 4294967295.
    \end{itemize}
    \item 6 literals, 0.0000000000001222\% of queries. Concretely: 
    \begin{itemize}
        \item ($2074+20470$) out of 18446744073709551615.
    \end{itemize}
    \item 7 literals, 0.00000000000000000000000000000003947\% of queries. Concretely: 
    \begin{itemize}
        \item ($8363+125940$) out of 340282366920938463463374607431768211455.
    \end{itemize}
    ...
    \item 12 literals,which hugely tends to 0\% of queries. Concretely: 
    \begin{itemize}
       \item ($2728+40920$) out of \\
    1797693134862315907729305190789024733617976978942306572734300811577326758055... \\ ...0096313270847732240753602112011387987139335765878976881441662249284743063947... \\ ...4124377767893424865485276302219601246094119453082952085005768838150682342462... \\ ...881473913110540827237163350510684586298239947245938479716304835356329624224137215
    \end{itemize}
\end{itemize}


Note that we are mixing both synthetic and industrial (the biggest ones) examples in these examples.





==> Appendices/8-algorithmsDepth.tex <==
\section{Algorithms unrolled}

Note the \textit{for} loop in the Alg~\ref{algoBruteForce} and the \textit{while} loop in Alg~\ref{algoModelLoop}.

%\begin{algorithm}
%\SetAlgoLined
%\textbf{Input: }$\phiT$\;
%$\varphi'\gets \phiT[l_i \leftarrow s_i]$;  \textit{VR} $\gets$ \{\}\;
%$\calC \gets \textit{choices}(\textit{literals}(\phiT))$;
%$\calR \gets 2^{\calC}$\;
%%$\textit{VR} \gets \emptyset$\;
% \For{$(P,A) \in \calR$}{
%   \If{$\exists\xs.\react_{(P,A)}(\xs)$ is valid}
%   {
%     $\textit{VR} \gets \textit{VR} \cup \{ (P,A) \}$\;
%    }
% }
% $\displaystyle\phiExtra \gets \bigwedge_{(P,A)\in \textit{VR}} (e_{(P,A)} \rightarrow \bigvee_{c\in P} (\bigwedge_{l_i\in c}s_i\wedge \bigwedge_{l_i\notin c}\neg s_i))$ \;
% $\phiB \gets \varphi' \wedge \phiExtra$ \;
% \Return $\phiB$
% \caption{Brute-force Boolean Abstraction algorithm}
% \label{algoBruteForce}
%\end{algorithm}

%\subsubsection{Model Loop algorithm} Note the \textit{while} loop.

%\begin{algorithm}[H] \label{algoModelLoop}
%\SetAlgoLined
%\textbf{Input: }$\phiT$\;
%$\varphi'\gets \phiT[l_i \leftarrow s_i]$;  \textit{VR} $\gets$ \{\}\;
%$\calC \gets \textit{choices}(\textit{literals}(\phiT))$;
%$\calR \gets 2^{\calC}$\;
% $\overline{c} \gets$ From  $\{\mathcal{C}, \mathcal{P}, \mathcal{A}\}$ obtain Boolean configurations, where $c \in \overline{c} \equiv p \in \mathcal{P}$ and $\neg c \in \overline{c} \equiv a \in \mathcal{A}$ \;
% $\varphi = \exists \overline{c} \textit{. } \neg(\bigwedge_{0 \leq i \leq |\overline{c}|} \neg c_i) $\;
% \While{$\textit{SAT}(\varphi)$}{
%    $m = model(\varphi)$\;
%    $t = translate\_toTheory(m)$\; %\#For instance, from $c_0 \neg c_1 \neg c_2 c_3$ to \textit{PAAP}. 
%    \If{$\exists \overline{x} :: (t)$ is valid}{
%    $pos = take\_Positives(t)$ \;
%    $\varphi = \varphi \wedge \neg(\bigwedge_{0 \leq j \leq |pos|} \neg pos_j)$ \;
%    \textit{VR} $\gets$ \textit{VR} $\cup$ $(e_{\textit{t}}, pots(t))$\;
%    %(i.e. Add: $fresh(\overline{e}) \implies Pots\_of(React_i)$) 
%    }
%    \Else{
%    $neg = take\_Negatives(t)$ \;
%    $\varphi = \varphi \wedge \neg(\bigwedge_{0 \leq k \leq |neg|} \neg neg_k)$ \;
%    }
% }
% $\displaystyle\phiExtra \gets \bigwedge_{(P,A)\in \textit{VR}} (e_{(P,A)} \rightarrow \bigvee_{c\in P} (\bigwedge_{l_i\in c}s_i\wedge \bigwedge_{l_i\notin c}\neg s_i))$ \;
% %$\varphi^{extra} \gets get\_minimal(\varphi^{extra})$ \;
% $\phiB \gets \varphi' \wedge \phiExtra$ \;
% \Return $\varphi^{\mathbb{B}}$
% \caption{Model-loop based Boolean Abstraction algorithm}
%\end{algorithm}

%\pagebreak

Note the heuristics in Alg. \ref{algoDefinitive}.

\begin{algorithm}[H] \label{algoDefinitive}
\SetAlgoLined
\textbf{Input: }$\phiT$\;
 \textit{fatigue}, \textit{division} \#These are (1) the fixed number of inner-loops and (2) if UNSAT outer model is divisible by this number, we enter inner-loop \;
 $\mathcal{S} \gets  get\_clusters(\textit{all\_literals})$ \;
 $\varphi^{extra} \gets \top$ \;
 \For{$s \in \mathcal{S}$}{
    $\varphi^{''} \gets \{\}$ \;
    $\overline{l} \gets get\_literals(\mathcal{S})$ \#Cluster's literals \;
    \For {$0<r<|\overline{l}|$}{
     $\varphi^{''} \gets \varphi^{''} \cup \varphi^{Num}[l_r \leftarrow s_r]$ \;
    }
     $\mathcal{C} \gets$ obtain\_the\_configutations\_from\_the\_literals\;
     $(\mathcal{P}, \mathcal{A}) \gets$ From $\mathcal{C}$, compute the sets of potentials and antipotentials \; 
     $\overline{c} \gets$ From  $\{\mathcal{C}, \mathcal{P}, \mathcal{A}\}$ obtain Boolean configurations, where $c \in \overline{c} \equiv p \in \mathcal{P}$ and $\neg c \in \overline{c} \equiv a \in \mathcal{A}$ \;
     Valid $\gets$ \{\}\;
     $num\_unsats \gets 0$ \;
     $\varphi = \exists \overline{c} \textit{. } \neg(\bigwedge_{0 \leq i \leq |\overline{c}|} \neg c_i) $\;
     \While{$\textit{SAT}(\varphi)$}{
        $t = translate\_toTheory(model(\varphi))$\;
        %$t = translate\_toTheory(m)$\; %\#For instance, from $c_0 \neg c_1 \neg c_2 c_3$ to \textit{PAAP}. 
        \If{$\exists \overline{x} :: (t)$ is valid}{
        $pos = take\_Positives(t)$ \;
        $\varphi = \varphi \wedge \neg(\bigwedge_{0 \leq j \leq |pos|} \neg pos_j)$ \;
        Valid $\gets$ Valid $\cup$ $(e_{\textit{t}}, pots(t))$\;
        %(i.e. Add: $fresh(\overline{e}) \implies Pots\_of(React_i)$) 
        }
        \Else{
        $neg = take\_Negatives(t)$ \;
        $\varphi = \varphi \wedge \neg(\bigwedge_{0 \leq k \leq |neg|} \neg neg_k)$ \;
        
            \If{$num\_unsats \% division = 0$}{
                $also\_cut = inner\_loop (t, \textit{fatigue})$ \; 
                $\varphi = \varphi \wedge \neg(\bigwedge_{0 \leq w \leq |also\_cut|} \neg also\_cut_w)$ \;
            }
        $num\_unsats = num\_unsats + 1$
        }
     }
 $\displaystyle \varphi^{extra}_s \gets \bigwedge_{(P,A)\in \textit{VR}} (e_{(P,A)} \rightarrow \bigvee_{c\in P} (\bigwedge_{l_i\in c}s_i\wedge \bigwedge_{l_i\notin c}\neg s_i))$ \;
     %$\varphi^{extra}_s \gets get\_minimal(\varphi^{extra}_s)$ \;
     $\varphi^{extra} = \varphi^{extra} \wedge \varphi^{extra}_s$
    }

 $\phiB \gets \varphi' \wedge \phiExtra$ \;
 \Return $\varphi^{\mathbb{B}}$
 \caption{Double SAT algorithm with heuristics}
\end{algorithm}


==> Appendices/8-extraOptimizations.tex <==
\section{Extra optimizations} \label{appSec:optimizations}

%We choose some basic heuristics that are combined. They are depicted in Alg.~\ref{algoDefinitive}.

\subsubsection{Main Antipotential core}

This heuristic consists of the following: once an outer model is obtained, it is asked whether the combination of all the antipotentials in conjunction is $\top$ or not (this is called the \textit{Main Antipotential Core}). If the Main core is $\perp$, then it is very likely that there exists an $\perp$ core that is a subcombination of the main one. On the other hand, if the main core is $\top$, then we already know (by logical argument) that we will not find $\perp$ cores purely composed of antipotentials, so the search for the inner loop is likely to be fruitless. Therefore, we enter the inner loop if and only if that Main core is $\perp$. 

For instance, let an outer loop model be $\textit{PAPA}$. If we query $\textit{?A?A}$ and we obtain $\perp$, then probably some subcombination (e.g., $\textit{???A}$) will be $\perp$, thus be an $\perp$ core. Else, if we obtained $\top$, then all the subcombinations will be $\top$, so there is no point in searching deeper.

We saw that using this heuristic, from a few outer models where the inner loop has been entered, in the following outer models the inner loops are hardly entered. The result is that the number of inner and outer models is balanced, producing much better times and number of queries.

%Note that the following two heuristics (and any other that is not explicitly mentioned) incorporate this heuristic, regardless of their internal parameters.

\subsubsection{Naive heuristics}

We have also proposed three very simple heuristics in order to balance the number of turns of the outer and inner loops; forcing, in particular, that there are more models in the outer loop

First, we have the fixed number of inner loops, which, as its name suggests, simply sets the maximum number of models that the inner loop can explore before cutting it and going to the next outer model. This idea is especially effective in (1) requirements with many literals, because the tree is larger to explore; and (2) the more outer models that have been already output, because more $\top$ results are likely to appear and thus explored in vain.

The second idea is that a division by module decides whether or not to enter the inner loop. Specifically, there is a counter for the number of times an $\perp$ model has been explored from the outer to the inner loop; the idea, then, is that when that number is divisible by another number that is chosen, only then the inner loop is entered. In this way, for example, only the $\perp$ that have come out in an even position are scanned.

The third idea is adding a decay over the quantity of times that we enter the inner loop. The reason fort this is that, (1) at the very beginning we extract a lot of information from each inner-loop, whereas (2) whenever the exploration moves forward, we get less information from it. Thus, we are interested in limiting the fuel used in inner loops, so we do it using a decay function. We implemented intuitive versions of this function, such as decreasing the fatigue in 1 unit for each 40 enters in inner-loops. Decays can also be discrete or continuous, but this is out of th escope of this paper.

\subsubsection{Preprocessing: Clustering}

This is a useful technique for reducing the size of the problem in a pre-processing-like phase.

To \textit{clusterize} the original requirements means making \textit{islands} of literals that share variables. If two islands do not share any variable, we can perform Boolean abstraction to them separatedly.

The algorithm for performing clustering is straightforward. All variables are traversed: for each (say $a$), its neighbours are stored; for the next variable (say $b$), if $a$ is a neighbour, then $b$ attaches not only the $a$ as a neighbour, but also all the neighbours of $a$. Thus, at the end we obtain $n \leq numVariable$ clusters that can be separatedly Booleanized.

For instance, given $\varphi = \square (((a>b) \implies (b>c)) \wedge ((e>f) \implies (d>g)) \wedge ((c>t) \implies (g>v))$, the algorithm Booleanized $(a>b) \implies (b>c))$ and $((c>t) \implies (g>v))$ on one process (since $c$ \textit{links} both clusters), and $((e>f) \implies (d>g))$ in another process. Then, both generated extra requirements are conjuncted.

==> Appendices/8-futureWork.tex <==
\section{Future work} \label{appSec:futureWork}

In this paper, we showed that if variables do not
relate over time then $\LTLt$ realizabilty is decidable (for $\exists^*\forall^*$-
decidable theories theories); however, it is easy to see that if one can relate variables
arbitrarily, we can build two counter machines (or TSL) to \textit{Super}$\LTLt$-realizability 
(proving undecidability). Thus, we are studying controlled (and useful) ways 
to pass information between temporal states; i.e., restricted forms of predicates
that relate variables accross time. This allows us to enrich TSL so that benchmarks that previously
were semi-decidable and hard to solve (e.g., experiment $5$ in \cite{maderbacherBloem2021reactiveSynthesisModuloTheoriesAbstraction}) 
become decidable and easily solvable expressed in $\LTLt$ and translated with Boolean Abstraction.
  
As for other ongoing challenges, they focus on the followings:

\begin{itemize}
    \item Enhancing the scalibility of the Boolean abstraction algorithm.
    Some of these optimizations rely on theory-based reasoning, whereas others
    exploit well-known decision procedures such as Cooper's quantifier
    elimination method~\cite{cooper1972theoremProving}.
    \item Expanding the expressive fragment of Boolean abstraction while maintaining decidability. 
    We are studiying its usage with non-arithmetic theories such as the 
    \textit{Theory of Arrays}~\cite{bradleyETAL2006whatDecidableAboutArrays}.
  \item Extending applicability of Boolean abstraction in different
    contexts.  For instance, Boolean abstraction can be used to
    pre-check the realizability of (rich) specifications to be used in monitors of runtime
    verification~\cite{gorostiagaSanchez2022hlolaVeryFunctionalStreamRV}.
\end{itemize}

Also, we are researching how to move from realizability modulo theories, to
(reactive) synthesis modulo theories, on realizable instances. The missing piece is 
the function that provides the system's values given environment's values that make 
the corresponding (Boolean) literals true. This function is guaranteed to exist, but 
we need to realize it as a computable function in some programming language.
%
Our early results are promising, and they suggest that this function can be obtained using an interplay 
between the algorithm that produces the extra formula and existential queries in SMT solvers.
However, we suspect there are ways to obtain more lightweight systems.

Note that Appendix~\ref{appSec:moreEmpirical} also contains interesting issues and work in progress
about empirical evaluation.

==> Appendices/9-newBenchmarking.tex <==
\section{Benchmarks in depth}

\subsection{Foundations}

We make use of other seven real industrial specifications in order to test the Boolean abstraction against problems of the industry; which also allows us to see patterns that recur when designing optimizations. These are these specification’s names \footnote{Note that we keep their names at minimum, and they have been altered in order not to reveal true industrial information. Also, note that they belong to different production areas whose particular usages are out of the scope of this article.}:

\begin{itemize}
    \item \textit{Lift}: This specification is part of a set of specifications that describes the functioning of a freight elevator system (see Appendix T1). It is composed of N requirements, it contains X literals and Y variables.
    \item \textit{Train}: This specification is part of a set of specifications describing the functioning of an autonomous train driving system (see Appendix T2). It is composed of N requirements, it contains X literals and Y variables.
    \item \textit{Connect}: This specification is part of a set of specifications describing the functioning of an electric vehicle charging and discharging system (see Appendix T3). It is composed of N requirements, it contains X literals and Y variables.
    \item \textit{Cooker}: This specification is part of a set of specifications describing the functioning of a system consisting of two independently operating liquid pumping tanks (see Appendix T4). It is composed of N requirements, it contains X literals and Y variables.
    \item \textit{Tanks}: This specification is part of a set of specifications describing the operation of a food processor with various functions (see Appendix T5). It is composed of N requirements, it contains X literals and Y variables.
    \item \textit{Usb}: This specification is part of a set of specifications describing the operation of a system that prevents the loss of information during the interaction between a USB and a machine (see Appendix T6). It is composed of N requirements, it contains X literals and Y variables.
    \item \textit{Stage}: This specification is part of a set of specifications describing the operation of a system that combines the use of different sensors for use in aviation (see Appendix T7). It is composed of N requirements, it contains X literals and Y variables.
\end{itemize}

Industrial specifications' literals can be found, as well as its clusters. Note that, as for industrial specifications.  the original ones belong to an enterprise \footnote{The company is: \url{https://www.developair.tech}} and, thus:

\begin{itemize}
    \item We add a short natural language description of what type of system has been requested (e.g., "this is a specification describing how a train behaves").
    \item We use only the literals we are interested in, i.e., the numerical ones, ignoring the original specification, temporality, Boolean variables etc (e.g., "$lit_1 = (x< 1000), lit_2 = (y >= z+1)$").
    \item We change the variable names, so that nothing is really intuited about the original specification (e.g., from '\textit{transistor\_voltage}' to '\textit{p}').
\end{itemize}

\subsubsection{Test by test}

\subsubsection{Industrial case 1: Lift}

This specification is part of a set of specifications that describes the functioning of a freight elevator system.

Concretely, different floors are selected on which to stop based on different weight parameters.

The full specification can be found in Appendix N, whereas the arithmetic/enumerated specification is the following:

//It is divided in clusters 1...

//As for cluster 1...

\subsubsection{Industrial case 2: Train}

This specification is part of a set of specifications describing the functioning of an autonomous train driving system.

Concretely, different sensors are read to know whether or not the doors can be closed after stopping at a station.

The full specification can be found in Appendix N, whereas the arithmetic/enumerated specification is the following:

//

\subsubsection{Industrial case 3: Connect}

This specification is part of a set of specifications describing the functioning of an electric vehicle charging and discharging system.

Concretely, different readings are obtained on the voltages of the load points to decide how to level the input and output power flow.

The full specification can be found in Appendix N, whereas the arithmetic/enumerated specification is the following:

//

\subsubsection{Industrial case 4: Two tanks}

This specification is part of a set of specifications describing the functioning of a system consisting of two independently operating liquid pumping tanks.

Concretely, it fluctuates between different heights in tank capacities, based on sensor readings of liquid flow rates.

The full specification can be found in Appendix N, whereas the arithmetic/enumerated specification is the following:

//

\subsubsection{Industrial case 5: Cooker}

This specification is part of a set of specifications describing the operation of a food processor with various functions.

Concretely, using internal information about the time and external information about the user, it varies between different cooking modes and intensities.

The full specification can be found in Appendix N, whereas the arithmetic/enumerated specification is the following:

//

\subsubsection{Industrial case 6: Usb}

This specification is part of a set of specifications describing the operation of a system that prevents the loss of information during the interaction between a USB and a machine.

Concretely, it features different security modes, as well as error handling and different possible connections between the USB and the machine.

The full specification can be found in Appendix N, whereas the arithmetic/enumerated specification is the following:

//

\subsubsection{Industrial case 7: Stages}

This specification is part of a set of specifications describing the operation of a system that combines the use of different sensors for use in aviation.

Concretely, it is shown how the readings of a pitot tube are managed, based on some resistor's temperatures, power voltages and tubes' altitude lectures.

The full specification can be found in Appendix N, whereas the arithmetic/enumerated specification is the following:

//


==> Minimal_paper/6-sota.tex <==
\section{State of the art} 

\subsubsection{Related work.}

Temporal Stream Logic~\cite{finkbeinerETAL2017temporalStreamLogicSynthesisBeyondBools}
extends LTL with complex data that can be related accross time, making use of a new 
\textit{update} operator; e.g., $\llbracket y \mapsfrom f x \rrbracket$ indicates that 
the result of applying function $f$ to variable $x$ is assigned to $y$.
%
This is later extended to theories in
\cite{finkbeinerETAL2021temporalStreamLogicModuloTheories,maderbacherBloem2021reactiveSynthesisModuloTheoriesAbstraction}.
%
In all these works, realizability is undecidable.
Also, in \cite{wonhyukETAL2022canSynthesisSyntaxBeFriends} reactive synthesis and SyGuS \cite{rajeevETAL2013syntaxGuidedSynthesis} collaborate in the synthesis process, 
and generate executable code that implements both reactive and data-level properties, thus
it suffers from two sources of undecidability: the undecidability of TSL synthesis \cite{finkbeinerETAL2017temporalStreamLogicSynthesisBeyondBools} 
and the undecidability of syntax-guided synthesis \cite{caulfieldETAL2015whatsDecidableAboutSyntaxGuidedS}.
%
In this paper, we cannot relate theory values accross time but we
prove that realizability is decidable for all LTL.

Constraint LTL
\cite{demriDSouza2002automataTheoreticApproachConstraintLTL} extends
LTL with the possibility of expressing constraints between variables
at bounded distance (of time).
%
The theories considered are a restricted form of $\ThZ$ with only
comparisons and the problem requires additional restrictions to
overcome undecidability.
%
In comparison, we do not allow predicates to compare variables at
different timesteps, but we prove decidability for all theories with an
$\exists^*\forall^*$ decidable fragment.

As for works closest to ours,~\cite{cheng2013numerical} proposes
numerical LTL synthesis using an interplay between an LTL synthesizer
and a non-linear real arithmetic checker.
%
However,~\cite{cheng2013numerical} overapproximates the
power of the system and not precise realizability.
%
Also, linear arithmetic games are studied in
\cite{azadehKincaid2017strategySynthesisLinearArithmetic} which
introduces algorithms for synthesizing winning strategies for
non-reactive specifications.

\subsubsection{TSL and $\textit{LTL}_{\mathcal{T}}$ are not comparable.}

%TSL original paper: https://arxiv.org/pdf/1712.00246.pdf
%TSL modulo theories: https://arxiv.org/pdf/1712.00246.pdf
%TSL SyGus (reviewer TACAS): https://www.wonhyuk.com/publications/pdf/pldi22.pdf 

When comparing TSL with $\LTLt$, note that $\LTLt$ includes all LTL,
whereas TSL is undecidable already for the theory of equality and Presburger arithmetic. Indeed,
TSL is undecidable for $T_U$, except for three fragments (see Thm. 7 in \cite{finkbeinerETAL2021temporalStreamLogicModuloTheories}):
it is (1) semi-decidable for the reachability fragment of TSL (i.e., the fragment of TSL
that only permits the next operator and the eventually operator as temporal
operators), it is (2) decidable for formulae consisting of only logical operators, predicates, updates, 
next operators, and at most one top-level eventually operator, 
and it is (3) semi-decidable for formulae with one cell (i.e., controllable outputs).

Thus, note that all the specifications considered for empirical evaluation in Sec~\ref{sec:empirical} 
are not decidable in TSL, since they are not within the considered decidable nor semi-decidable fragments. 
Also, note that TSL allows (finite) uninterpreted predicates, whereas we need to have predicates
well defined within the semantics of theories of specifications for which we perform Boolean abstraction.

%\subsubsection{Comparing $\textit{LTL}_{\mathcal{T}}$ to TSL} //The key is the update statement: show e.g., elevator.

%\subsubsection{Comparing $\textit{LTL}_{\mathcal{T}}$ to CTL} //No idea

%\subsubsection{Comparing $\textit{LTL}_{\mathcal{T}}$ to MLTL and STL} //No idea

==> Minimal_paper/7-supportMaterial.tex <==
\section{Enriching material}

\subsection{Showing tree pruning of Double-SAT method} \label{subsec:pruning}

We explore the results of the Double-SAT method in a 2 literal example, where we set fatigue (i.e., maximum inner-loop models) at 3 and a decay of 1 (i.e., it decreases 1 per each explored outer-model). The execution is as follows:

\begin{enumerate}
    \item Model \textit{PAAP} is obtained. Since it is invalid, we look for $\textit{fatigue}=3$ $\perp$ cores: obtaining \textit{PA??}, \textit{??AP} and \textit{?AA?}. Thus, we eliminate \textit{PPAP} and \textit{PAPP} above; \textit{PAPA} and \textit{APAP} at the same level; and \textit{PAAA} and \textit{AAPA} below.
    \item  Model \textit{PPAA} is obtained. Since it is valid, we eliminate \textit{PPPA} and \textit{PPPP} above as uninteresting cases.
    \item Model \textit{AAPP} is obtained. Since it is valid, we eliminate \textit{APPP} above as an uninteresing case.
    \item Model \textit{APPA} is obtained. Since it is invalid, we look for $\textit{fatigue}-decay=3-1=2$ $\perp$ cores: \textit{AP??} and \textit{??PA}. Thus, we eliminate \textit{APAA} and \textit{AAPA} below.
\end{enumerate}

\begin{figure}[h!]
	 \centering
      \includegraphics[width=0.75\linewidth]{Figs/test1_DoubleSAT.png}
      \caption{An execution of the double-SAT-based-loop algorithm over
        the running example. The rounded reactions where returned by
        the SAT solver, with a tick if they are valid reactions and
        cross if they are not. Crossed-out reactions mean that they
        have been derived to be uninteresting or invalid by findings on X reaction. Note that the all-antipotentials case \textit{AAAA} is already $\perp$ (thus, unexplored).
}
      \label{figDoubleSAT}
\end{figure}

This execution has performed 4/15 SAT+SMT queries in the outer loop, and 3+2 SAT+SMT queries in the inner loops. This yields 9 SAT+SMT queries out of the total of 16 \footnote{Or 15, but $\perp$ cores would also discover invalidity of \textit{AAAA})}.

This (convenient) example shows how a proper heuristic-setup of fatigue, decay etc makes a search shorter. This is much more useful with long benchmarks.

\subsection{Industrial table} \label{subsec:industrial}

We can see results cluster by cluster. Note that each of them has a different heuristic-setup.

%Note that all of them are fixed in the best heuristic-setup, i.e., $\textit{fatigue}=30$ as the maximum inner-loop and 2 as the modulo division. %, except for $Cl_3$ and $Cl_4$ in \textit{Lift}, which are fixed with maximum inner-loop of 5 and 3 respectively (no strong reasong for that).
%
%Note that fatigue's decay is sometimes used.% (i.e., $f(decay, \textit{fatigue})=\textit{fatigue}$).
%Also, a fatigue decay has been used: $fatigue=fatigue-1$ for every 100 times the inner loop is entered.

\TableBenchmark

\subsection{(Short) Related work}

At \cite{finkbeinerETAL2021temporalStreamLogicModuloTheories,maderbacherBloem2021reactiveSynthesisModuloTheoriesAbstraction}, they Temporal Stream Logic \cite{finkbeinerETAL2017temporalStreamLogicSynthesisBeyondBools} is extended with first-order theories, but $\textit{TSL}_{\mathcal{T}}$ satisfiability is highly undecidable, while our approach is decidable. Also, in Constraint LTL
\cite{demriDSouza2002automataTheoreticApproachConstraintLTL}, LTL is extended with the possibility of expressing constraints between variables
at bounded distance (of time).
%
The difference with respect to this paper is that we do not allow
any type of predicate of variables within
different timesteps.

As for works closest to ours, the \cite{cheng2013numerical} preprint
proposes a numerical LTL synthesis, whose
calculations involve an interplay between an LTL synthesizer and a
non-linear real arithmetic theory checker. However, their idea only
considers specifications where the arithmetic predicates belong to the
environment, and indeed they \textit{overapproximate} the result.
%

Also, the problem of solving linear arithmetic games is addressed in
\cite{azadehKincaid2017strategySynthesisLinearArithmetic}, producing
algorithms for synthesizing winning strategies. However,
in addition to not being a Booleanization method, but a synthesis
method, they do not consider time modalities either.

To finish, a witness of a recent researches on infinite-state-games is 
is \cite{baier2021causalitybased}.

\begin{comment}
    
\pagebreak

\begin{center} \label{tablLift}
\begin{tabular}{| c || c | c | c ||} 
 \hline
 Benchmark & Cluster (vars / lits) & Time (s) & Queries (outer / inner) \\ [0.5ex] 
 \hline\hline
 \multirow{4}{*}{\textit{Lift}} & $Cl_1$ (1, 7) & 32.38 &  60 / 900 \\ 
 & $Cl_2$ (2, 4) & 1.27 &  16 / 30 \\
 & $Cl_3$ (1, 3) & 0.57 &  10 / 10\\
 & $Cl_4$ (1, 2) & 0.23 &  4 / 3 \\
 \hline\hline
 \multirow{8}{*}{\textit{Train}} & $Cl_1$ (1, 3) & 1.51 &  26 / 58 \\ 
 & $Cl_2$ (2, 1) & 0.06 &  2 / 0 \\
 & $Cl_3$ (1, 3) & 0.29 &  2 / 13 \\
 & $Cl_4$ (1, 1) & 0.14 &  3 / 2 \\
 & $Cl_{5.1}$ (3, 6) & 833.32 &  1620 / 9199 \\
 & $Cl_{5.2}$ (4, 6) & 4749.05 &  11604 / 166050 \\
 & $Cl_{6.1}$ (3, 5) & 1377.67 &  3915 / 55770 \\
 & $Cl_{6.2}$ (3, 12) & 6571.97 &  2728 / 40920 \\
 \hline\hline
 \textit{Connect} & $Cl_{\textit{unique}}$ (2, 2) & 0.12 &  4 / 0 \\ 
 \hline\hline
 \textit{Cooker} & $Cl_{\textit{unique}}$ (3, 5) & 2.82 &  8 / 120 \\ 
 \hline\hline
 \multirow{2}{*}{\textit{Usb}} & $Cl_{\textit{unique}}$ (2, 3) & 0.26 &  8 / 0 \\ 
 & $Cl_{\textit{modification}}$ (3, 5) & 1390.75 &  18038 / 0 \\ 
 \hline\hline
 \multirow{2}{*}{\textit{Stage}} & $Cl_A$ (8, 8) & 34.25 &  256 / 0 \\ 
 & $Cl_B$ (8, 11) & 2895.74 &  25216 / 2790 \\
 \hline
\end{tabular}
\end{center}

\pagebreak

\begin{center} \label{tablLift}
\begin{tabular}{| c ||| c ||| c | c | c || c | c | c || c | c | c | c |} 
 \hline
 Benchmark & Cluster & \multicolumn{3}{|c||}{Time (s) } & \multicolumn{3}{|c||}{Queries (out+inn)} & \multicolumn{4}{|c|}{Heuristics (double-SAT)} \\ 
 %\multirow{2}{*}{(name)} & \multirow{2}{*}{(vars / lits)} & \multicolumn{3}{c}{(s)} & \multicolumn{3}{c}{(outer / inner)} & \multicolumn{4}{c}{(of double SAT)} \\
 \cline{3-12}
  (name) & (vars, lits) & BF & SAT & Double & BF & SAT & Double & Max-Inner & Modulo & Decay & U-core \\ [0.5ex] 
 \hline\hline
 \multirow{4}{*}{\textit{Lift}} & $Cl_1$ (1, 7) & $\perp$ & E & \textbf{32.38} &  E & E & \textbf{60/900} & a & b & c & $\checkmark$ \\ 
 & $Cl_2$ (2, 4) & E & E & \textbf{1.27} &  E & E & \textbf{16/30} & a & b & c & $\times$\\
 & $Cl_3$ (1, 3) & E & E & \textbf{0.57} &  E & E & \textbf{10/10} & a & b & c & d \\
 & $Cl_4$ (1, 2) & E & E & \textbf{0.23} &  E & E & \textbf{4/3} & a & b & c & d \\
 \hline \hline
  \multirow{8}{*}{\textit{Train}} & $Cl_1$ (1, 3) & E & E & \textbf{0.09} &  E & E & \textbf{6/55}  & 100 & 20 & 40 & $\times$ \\ 
 & $Cl_2$ (2, 1) & E & E & \textbf{0.04} &  E & E & \textbf{2/0} & 100 & 20 & 40 & $\times$\\
 & $Cl_3$ (1, 3) & E & E & \textbf{0.24} &  E & E & \textbf{2/13} & 100 & 20 & 40 & $\times$ \\
 & $Cl_4$ (1, 1) & E & E & \textbf{0.08} &  E & E & \textbf{3/2} & 100 & 20 & 40 & $\times$ \\
 %& $Cl_{5.1}$ (3, 6) & $\perp$ & E & \textbf{833.32} & E & E & \textbf{1620/9199} & a & b & c & $\checkmark$ \\ 
  & $Cl_{5.1}$ (3, 6) & $\perp$ & E & \textbf{102.46} & E & E & \textbf{1778/2960} & a & b & c & $\times$ \\ 
 %& $Cl_{5.2}$ (4, 6) & E & E & \textbf{4749.05} &  E & E & \textbf{11604/166050} & a & b & c & $\times$\\
 & $Cl_{5.2}$ (4, 6) & E & E & \textbf{4890.21} &  E & E & \textbf{60355/6545} & a & b & c & $\times$\\
 %& $Cl_{6.1}$ (2, 4) & E & E & \textbf{1377.67} &  E & E & \textbf{3915/55770} & a & b & c & $\times$ \\
  & $Cl_{6.1}$ (2, 4) & E & E & \textbf{564.90} &  E & E & \textbf{12022/10302} & a & b & c & $\times$ \\
 & $Cl_{6.2}$ (3, 12) & E & E & \textbf{6571.97} &  E & E & \textbf{2728/40920} & a/b & b & c & $\times$ \\
 \hline \hline
 \textit{Connect}& $Cl_1$ (2, 2) & E & E & \textbf{0.12} & E & E & \textbf{4/0} & a  & b & c & d \\
  \hline \hline
 \textit{Cooker}& $Cl_1$ (3, 5) & E & E & \textbf{2.82} &  E & E & \textbf{8/120} & a/b  & b & c & d \\
 \hline \hline
\multirow{2}{*}{\textit{Usb}} & $Cl_1$ (2, 3) & $\perp$ & E & \textbf{0.26} & E & E & \textbf{8/0} & a & b & c & $\checkmark$ \\ 
 & $Cl_2$ (3, 5) & E & E & \textbf{1390.75} &  E & E & \textbf{18038}  & a & b & c & $\times$\\
 \hline \hline
  \multirow{2}{*}{\textit{Stage}} & $Cl_1$ (8, 8) & $\perp$ & E & \textbf{34.25} &  E & E & \textbf{256/0} & a & b & c & $\checkmark$ \\ 
 & $Cl_2$ (8, 11) & E & E & \textbf{2895.74} & E & E & \textbf{25216/2790}  & a & b & c & $\times$\\
 \hline
\end{tabular}
\end{center}

\end{comment}


%//Maybe we can further explore these results.

%//We can also add the synthetic table and talk more about it.

%//Or we can mention Tanks and how we do not know how to solve it: then, we could mention there are some techniques being developed... (CAV)

%//We can also try to make the algorithm below shorter. Or maybe do not include it and only leave Algorithm Skeleton in main paper, whereas Algorithm brute force, SAT and double-SAT (with optimizations) are in the Appendices.

==> Minimal_paper/results_Realizability.tex <==
\newcommand{\TableBenchmarkRealizability}{
\begin{figure}[b!]
%  \centering
\begin{tabular}{|c|c|c|c||c|c|c|c||c|c|c|}  \hline
  \multicolumn{4}{|c||}{Description of $\phiT$} & \multicolumn{4}{|c||}{Generated $\phiB$} & \multicolumn{3}{|c|}{Realizability.} \\ 
 \cline{1-11}
  Ben. & Clus. & R/U & Size & Alg. & Heur. & Size. & Reacts. & Abs. & Str. & LTL. \\ [0.5ex] 
 \hline\hline
 \multirow{4}{*}{\textit{Li.}} & (1, 7) & $\perp$ & 6740.23 & \textbf{31.77} & 30375 & \textbf{72/1040} & 16 & 2 & 0 & $\checkmark$ \\ 

 & (2, 4) & 3911.85 & \textbf{0.70} & 0.91 & \textbf{27} & 25/20 & 10 & 2 & 0 & $\times$ \\
 & (1, 3) & 3.64 & 1.19 & \textbf{0.52} & 46 & \textbf{10/20} & 10 & 2 & 0 & $\times$ \\
 & (1, 2) & 0.23 & \textbf{0.09} & 0.14 & 4 & \textbf{4/3} & 3 & 3 & 0 & $\times$ \\
 \hline \hline
  \multirow{8}{*}{\textit{Tr.}} & (1, 3) & $3.18$ & \textbf{0.04} &  0.96 & \textbf{16} & 26/20  & 10 & 2 & 0 & $\checkmark$ \\ 
 & (2, 1) & $0.05$ & \textbf{0.04} & \textbf{0.04} & \textbf{2/0} & \textbf{2/0} & 1 & 1 & 0 & $\checkmark$\\
 & (1, 3) & $3.10$ & 1.64 & \textbf{0.21} & $74$ & \textbf{2/10} & 10 & 2 & 0 & $\checkmark$ \\
 & (1, 1) & \textbf{0.04} & 0.06 & 0.11 & \textbf{3} & 3/2 & 1 & 1 & 0 & $\checkmark$ \\
    & (3, 6) & $\perp$ & 1269.45 & \textbf{112.58} & 13706 & \textbf{1170/4716} & 100 & 20 & 40 & $\times$ \\ 

 & (4, 5) & $\perp$ & $5251.09$ & \textbf{4144.89} & \textbf{44177} & 52623/12332 & 100 & 20 & 40 & $\times$\\
  & (3, 5) & $\perp$ & 2044.00 & \textbf{359.37} & 31363 & \textbf{9123/10158} & 100 & 20 & 40 & $\times$ \\
 & (4, 12) & $\perp$ & $\perp$ & \textbf{6571.97} & $\perp$ & \textbf{2728/40920} & 100 & 20 & 40 & $\times$ \\
 \hline \hline
 \textit{Con.}& (2, 2) & 0.23 & \textbf{0.09} & \textbf{0.09} & \textbf{4} & \textbf{4/0} & 3 & 3 & 0 & $\checkmark$ \\
  \hline \hline
 \textit{Coo.}& (3, 5) & $\perp$ & 1356.64 & \textbf{2.81} & 27883 & \textbf{16/160} & 20  & 2 & 0 & $\checkmark$ \\
 \hline \hline
\multirow{2}{*}{\textit{Usb}} & (2, 3) & $3.40$ & 0.21 & \textbf{0.17} & \textbf{8} & \textbf{8/0} & 3 & 3 & 0 & $\checkmark$ \\ 
& (3, 5) & $\perp$ & \textbf{231.94} & 364.46 & \textbf{5638} & \textbf{5638/0}  & 20 & 2 & 0 & $\checkmark$\\
 \hline \hline
  \multirow{2}{*}{\textit{St.}} & (8, 8) & $\perp$ & \textbf{18.19} & 18.20 & \textbf{256} & \textbf{256/0} & 40 & 2 & 0 & $\checkmark$ \\ 
 & (3, 6) & $\perp$ & 1311.32 & \textbf{194.83} & 14994 & \textbf{1697/6536}  & 100 & 20 & 40 & $\times$\\
 \hline \hline
   \multirow{7}{*}{\textit{Syn.}} & (2, 2) & 0.21 & 0.24 & \textbf{0.18} & 11 & \textbf{4/3}  & 3 & 3 & 0 & $\checkmark$ \\ 
 & (2, 3) & 3.42 & 2.69 & \textbf{1.24} & 119 & \textbf{14/40} & 10 & 2 & 0 & $\checkmark$\\
 & (2, 4) & $2842.97$ & 108.61 & \textbf{16.51} & 3982 & \textbf{188/620} & 10 & 2 & 0 & $\checkmark$ \\
 & (2, 5) & $\perp$ & $7151.03$ & \textbf{68.90} & $44259$ & \textbf{380/2800} & 20 & 2 & 0 & $\checkmark$ \\
  & (2, 6) & $\perp$ & $\perp$ & \textbf{402.27} & $\perp$ & \textbf{4792/9941} & 100 & 20 & 40 & $\times$ \\  
  & (2, 7) & $\perp$ & $\perp$ & \textbf{3596.71} & $\perp$ & \textbf{7344/139440}  & 40 & 2 & 0 & $\checkmark$ \\
  & (2, 7) & $\perp$ & $\perp$ & \textbf{3862.89} & $\perp$ & \textbf{24311/40615}  & 200 & 20 & 40 & $\times$ \\
 \hline

\end{tabular}
\caption{Empirical evaluation results on realizability of specifications generated by Boolean abstraction algorithms.}
  \label{tab:benchmarkRealizability}
  % \end{table}
\end{figure}
}
